URL: Universal Referential Knowledge Linking via Task-instructed Representation Compression

Linking a claim to grounded references is a critical ability to fulfill human demands for authentic and reliable information. Current studies are limited to specific tasks like information retrieval or semantic matching, where the claim-reference relationships are unique and fixed, while the referential knowledge linking (RKL) in real-world can be much more diverse and complex. In this paper, we propose universal referential knowledge linking (URL), which aims to resolve diversified referential knowledge linking tasks by one unified model. To this end, we propose a LLM-driven task-instructed representation compression, as well as a multi-view learning approach, in order to effectively adapt the instruction following and semantic understanding abilities of LLMs to referential knowledge linking. Furthermore, we also construct a new benchmark to evaluate ability of models on referential knowledge linking tasks across different scenarios. Experiments demonstrate that universal RKL is challenging for existing approaches, while the proposed framework can effectively resolve the task across various scenarios, and therefore outperforms previous approaches by a large margin.

==> figures/api_ins.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{figures/api_ins.pdf} 
\caption{Scores of text-embedding-3-large with or without task-aware instructions. It shows that directly using task-aware instructions will damage performance of api.}
\label{fig:api_ins}
\end{figure}

==> figures/arg_top.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{figures/arg_top.pdf} 
\caption{Scores under different ndcg@n setting. All the models perform better with larger n, and our Adaptive Embedding always up-performs the others.}
\label{fig:arg_top}
\end{figure}

==> figures/ceval.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{fig/ceval.pdf} 
\caption{Results of LLM retrievers in C-Eval. We compare three kinds of LLM retrievers in four evaluation datasets in C-Eval. The left is to let LLM generate correct answer based on question and calculate language model loss, the right is to calculate rate of failing the question when choosing correct choice via embedding similarity. We show multi-level method is lower than contrastive learning in both situation. This means that our method need less "alignment tax" when aligning LLM to dense retrieval tasks.}
\label{fig:ceval}
\end{figure}

==> figures/error.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{figures/error.pdf} 
\caption{Statistics of datas that URL can correctly handle but other models fail. The w/o g. means finetuning the LLM without the generative reconstruction.}
\label{fig:error}
\end{figure}

==> figures/eval_data.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures/eval_data.pdf} 
\caption{Illustration of URLBench. In actual scenarios, these four tasks are about making stock decision, legal judgment, medical prescription and college course planning. The benchmark greatly reflects the challenge of RKL.}
\label{fig:eval_data}
\end{figure*}

==> figures/eval_method.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.8\linewidth]{figures/eval_method.pdf} 
\caption{Generating task-aware embedding. Pooling last-layer hidden states of suffix tokens to get it.}
\label{fig:eval_method}
\end{figure}

==> figures/ppl.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{fig/ppl.pdf} 
\caption{The processing of multi-level alignment.}
\label{fig:ppl}
\end{figure}

==> figures/train_data.tex <==
% 这个东西属实有点丑，这个图的目的是说明我标注的数据涵盖了很多领域，好像也不是很关键这个问题
\begin{figure}[t!]
\centering
\includegraphics[width=0.8\linewidth]{fig/train_data.pdf} 
\caption{Domains in our 1000 train data. We totally annotate 40 domains. We annoate domain instructino and domain prompt for each doimain. These instructino and promp are used as in figure~\ref{fig:method}.}
\label{fig:train_data}
\end{figure}

==> figures/train_encoder.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{fig/train_encoder.pdf} 
\caption{Results of average recall scores of four datasets. We train nine baseline models via our 1000 training datas, compared with original models, some are better and some are worse, but all of them perform worse than our multi-level aligned LLM retriever. This means the reason why these bert-type retrievers can not do well is not related with  training data.}
\label{fig:train_encoder}
\end{figure}



==> sections/introduction_.tex <==
\section{Introduction}

% 背景
Access to reliable and well-founded information is a fundamental human need~\cite{clifford1877ethics, cole2011theory}. In recent years, there are increasing demands to locate corresponding documentations and validate the authenticity of information, particularly after the rise of AI generated content~\cite{gao2023retrievalaugmented, cao2023comprehensive}. % 总述大背景
In this process, an important component is linking a claim to its grounded references, referred to as referential knowledge linking (RKL). % RKL的任务定义
For a claim, the references from reliable information source can be used to do validating, supporting,  judging etc.~\cite{yue2023disclawllm, huang2023survey}. Therefore, RKL plays a crucial role in confirming the accuracy of information, increasing the reliability of intelligence, and ensuring the authenticity of AI generated content. % 展开到RKL的重要作用


\input{figures/domain}
\input{figures/method}
\input{figures/eval_method}
% 问题
Currently, works on RKL are often limited to tasks with simple and single claim-reference relationship. % 总述RKL的现状
For instance, semantic matching is to identify two sentences with same meaning, the core of this task is to handle \textit{semantic overlapping}~\cite{cer-etal-2017-semeval, 10.1145/3440755}. Similarly, information retrieval focuses on finding documents that contain information for a given query, the essence of this task is to handle \textit{informational overlapping}~\cite{10184013, muennighoff2023mteb}. % 论据
However, RKL is much more complex in real-world scenarios, because claims and references are heterogeneous, and relationships are knowledge-rich and versatile. % 总述当前研究与现实应用之间的gap
As illustrated in Figure~\ref{fig:domain}, given a legal case, we link it to corresponding provisions to find the basis for judging. Similarly, given a patient symptom, we link it to relevant drugs, treatment plans, or possible cause, depending on the specific need. % 论据


% 问题的挑战和价值
Addressing real-world RKL tasks is valuable and also challenging because of the versatile and knowledge-rich feature, and possible large computation. % 总述挑战
First, the claim-reference relationship is heterogeneous and dynamic although RKL tasks are with same pattern. Even more challenging, whether a claim and a reference form a linking pair is inconsistent under different situations. % 挑战一（多样性）：总述
For instance, given a legal case and a provision, it can get completely different linking decisions under the conditions "applying for adults" or "applying for minors". % 挑战一（多样性）：论据
Second, many RKL tasks require deep knowledge, understanding, and reasoning to link the claim and reference, rather than simple informational or semantic overlapping as in information retrieval and semantic matching tasks. % 挑战二（知识）：总述
For instance, given a training objective (claim) about "IT Engineer", the course (reference) about "Complex Function" is a basic supporting for the objective. But this claim-reference pair seems nearly unrelated on the surface semantic, thus requires great knowledge and reasoning capabilities. % 挑战二（知识）：论据
Additionally, it is inefficient to directly perform complex and deep-level interaction on all claim-reference pairs, because reference libraries are usually in extensive size. % 挑战三（效率）
In summary, it is important and challenging to construct an efficient, highly adaptable model with powerful knowledge and reasoning abilities. % 总结挑战和价值


% 方法的思路
In this paper, we propose Adaptive Embedding, a novel framework based on Large Language Models (LLMs) aimed at universal RKL. % 总述思路
Specifically, our motivation is to leverage general powerful reasoning and instruction-following capabilities of LLMs to achieve universal performance in RKL across various scenarios. % 展开
However, applying LLMs to RKL still presents many challenges due to characteristics of LLMs and the task pattern of RKL. % 总述思路上的困难
First, the performance of LLMs can be limited if they are not explicitly made aware of facing scenarios and tasks. % 困难一（需要让模型识别任务场景）
Second, direct pairwise comparison by LLMs is highly inefficient, due to the high computational cost of LLMs and large scale of reference libraries. % 困难二（效率）
Most importantly, directly applying LLMs for RKL can lead to a bad performance, because LLMs are originally trained by next-token prediction loss, there needs some suitable training to align LLMs to RKL. % 困难三（对齐到linking任务上）
In summary, addressing these key challenges is central to harnessing powerful abilities of LLMs for universal RKL. % 总结思路上的困难


\input{figures/eval_data}
% 方法的实现
To this end, we implement the framework by task-aware embeddings based on multi-view finetuning LLMs.  % 总述
As shown in Figure~\ref{fig:method}, this approach combines the claim and reference with task-aware instructions, then converts them into task-aware embeddings. As a result,  representations of the claim and reference can adapt to various RKL situations. % 对困难一（需要实现task-aware）的回应
Based on mentioned task-aware embeddings, linking becomes much more efficient. We can directly measure the similarity between embeddings, this relieves the complex interaction between claim-reference pairs, thus significantly enhance the efficiency of RKL. % 对困难二（效率）的回应
To get such an embedder suitable for universal RKL, we propose a  multi-view training method.  % 对困难三（对齐到linking任务上）的回应：总述
Specially, we finetune the LLM by jointing generative learning and contrastive learning, which aims at enhancing task-aware embeddings for the claim and reference. This jointing method compresses capabilities of the LLM into task-aware embeddings, and adapts embeddings with the pattern of RKL. % 对困难三（对齐到linking任务上）的回应：展开
Furthermore, we propose a method to construct training datas by transforming normal question-answer pairs into RKL datas.  % 对困难三（对齐到linking任务上）的继续回应：总述
Specially, we annotate task-aware instructions for each question-answer pair based on the field of this pair. And we use question-answer datas in heterogeneous fields to simulate versatile RKL tasks. This is an efficient solution in the situation that absents real versatile RKL training datas. % 对困难三（对齐到linking任务上）的继续回应：展开


% benchmark
Finally, we construct a new benchmark named RKLB to make up the deficiency of RKL evaluation. RKLB is collected from various real-world scenarios, thereby can greatly evaluate the ability of models in generalized RKL. % 总述evaluation benchmark
Specifically, RKLB covers four distinct domains: finance, law, medicine, and education. In these domains, RKLB requires models to link claims to references under various situations, which primarily includes linking government policy to company profile, legal case to legal provision, patient symptom to drug description, and training objective to course introduction. % 展开

% 结论
Experiment results on RKLB indicate that our framework is an effective approach for universal RKL. % 总述
Adaptive Embedding not only surpasses models trained on extensive retrieval datas but also significantly exceeds powerful large-scale embedding models such as OpenAI text embedding in most evaluation. This confirms the universal and advanced effectiveness of Adaptive Embedding. % 展开

The main contributions of this paper are:

$\bullet$~We define the task of referential knowledge linking, considering linking in a universal perspective, surpassing existing works that focus on the simple and single claim-reference relationship.

$\bullet$~We propose a novel framework for universal referential knowledge linking, which involves generating adaptive embeddings, constructing training datas, and employing multi-view finetuning.

$\bullet$~We construct a new benchmark across versatile knowledge-rich tasks in various fields, which can effectively reflect the challenge of referential knowledge linking in real-world scenarios.

==> tables/case.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{ll}
    \toprule
    \textbf{Claim} & This major focuses on systematic mastery of \textbf{robot engineering} ... \\
    \midrule
    \textbf{Reference} & This course is to introduce the methods of \textbf{feedback control} systems ... \\
    \toprule
    \textbf{Claim} & This major focuses on systematic mastery of robot engineering ... \\
    \midrule
    \textbf{Reference} & This major focuses on systematic mastery of robot engineering ... \\
    \bottomrule
    \end{tabular}%
}
\caption{}
\label{tab:case}%
\end{table}%


% \textit{Claim}: 

% \textit{Easy Reference}: This course aims to develop students' abilities in robot kinematics and ...

% \textit{Challenging Reference}: 

==> tables/error_2.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
    \toprule
    \textbf{Type} & \textbf{URL\cmarkgreenb~BGE\cite{xiao2023cpack}\xmarkredb} & \textbf{URL\cmarkgreenb~Only Contrastive learning\xmarkredb} \\
    \midrule
    Challenging & 75\% & 82\% \\
    Shallow & 25\% & 18\% \\
    \bottomrule
    \end{tabular}%
}
\caption{Two categories of cases that URL can handle correctly but other methods can not, which are claim-reference pairs requiring challenging knowledge or shallow knowledge. In these cases, the proportion of challenging data is far greater than shallow datas.}
\label{tab:error}%
\end{table}%

==> tables/eval_data.tex <==
% 这个sentence1 sentence2怎样命名比较好呢？
% 到时候记得把这个表格填的满一些
\begin{table*}[t]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{m{1.5cm}m{6.5cm}m{6.5cm}}
\hline
\textbf{Domain} & \textbf{Sentence 1} & \textbf{Sentence 2} \\
\hline
    & \textbf{Government policy} & \textbf{Company profile} \\
finance &
Key efforts will be made to promote the mass production and application of core equipment such as lithography machines, etching machines, ion implantation machines, and epitaxial furnaces ... & 
The company is a key equipment supplier in the fields of metal injection molding (MIM) and wide band-gap semiconductors, with material research as the foundation and high-temperature thermal ... \\ 
\hline
    & \textbf{Legal case} & \textbf{Legal provision} \\
law &
The plaintiff Xie Wenqiang filed a lawsuit claiming that on September 6, 2011, the defendant Lin Wei borrowed RMB 100000 from the plaintiff, with an agreed monthly interest rate of 8 cents ... & 
The loan contract shall be in written form, except as otherwise agreed between natural persons. The content of the loan contract includes terms such as the type of loan, currency, purpose, amount ... \\ 
\hline
    & \textbf{Patient symptom} & \textbf{Drug description} \\
medical &
Last night, my whole body was cold and I had no strength in my limbs. I haven't had an appetite all day today and don't want to eat anything.  There are no symptoms of abdominal pain or diarrhea ... & 
Compound paracetamol and amantadine capsules are suitable for relieving fever, headache, limb pain, sneezing, runny nose, stuffy nose, sore throat and other symptoms caused by common cold and influenza ... \\ 
\hline
    & \textbf{Train objective} & \textbf{Course introduction} \\
education &
Mastering solid theoretical and professional knowledge in computer science and technology, possessing the ability to analyze and solve problems, And the ability to self update knowledge  ... & 
The course of Mathematical Analysis helps students understand and master the theories related to real numbers, real number sequence theory, function limit theory, continuous function theory ... \\ 
\hline
\end{tabular}
\end{adjustbox}
\caption{Examples of datasets across four actual situation. When evaluate, given sentence 1, let retriever match correct sentence 2. In real situation, these four are about making stock decision, legal case judgment, medical prescription or college course plan. Note that our benchmark is more challenge for retriever because the pair do not have too much semantic overlapping, thus need retrievers do some reasoning, detailed analysis is in section~\ref{sec:5.1}.}
\label{tab:eval_data}
\end{table*}



==> tables/eval_instruction.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{m{16cm}}
    \toprule
    \textbf{Task-awareness instructions for claim:}  Above text is description of a \{government policy / legal case / patient symptom / training objective\}. Based on your own knowledge, compress it into an embedding that can be used to search for relevant \{company profile / legal provision / drug description / course introduction\}. The embedding is: \\
    \midrule
    \textbf{Task-awareness instructions for reference:}  Above text is a \{company profile / legal provision / drug description / course introduction\}. Based on your own knowledge, compress it into an embedding that can be used to match relevant \{government policy / legal case / patient symptom / training objective\}. The embedding is: \\ 
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{Examples of task-aware instruction. It contains description of the scenario and the using of the embedding.}
\label{tab:eval_instruction}
\end{table*}


==> tables/prompt.tex <==
\begin{table*}[t!]
\centering
\begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{m{16cm}}
    \toprule
    \textbf{Task-awareness instructions for claim:}  Above text is description of a \{government policy / legal case / patient symptom / training objective\}. Based on your own knowledge, compress it into an embedding that can be used to search for relevant \{company profile / legal provision / drug description / course introduction\}. The embedding is: \\
    \midrule
    \textbf{Task-awareness instructions for reference:}  Above text is a \{company profile / legal provision / drug description / course introduction\}. Based on your own knowledge, compress it into an embedding that can be used to match relevant \{government policy / legal case / patient symptom / training objective\}. The embedding is: \\ 
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{Examples of task-aware instruction. It contains description of the scenario and the using of the embedding.}
\label{tab:eval_instruction}
\end{table*}

